Inference in Sparse Graphs with Pairwise Measurements and Side Information

We consider the statistical problem of recovering a hidden "ground truth" binary labeling for the vertices of a graph up to low Hamming error from noisy edge and vertex measurements. We present new algorithms and a sharp finite-sample analysis for this problem on trees and sparse graphs with poor expansion properties such as hypergrids and ring lattices. Our method generalizes and improves over that of Globerson et al. (2015), who introduced the problem for two-dimensional grid lattices. For trees we provide a simple, efficient, algorithm that infers the ground truth with optimal Hamming error has optimal sample complexity and implies recovery results for all connected graphs. Here, the presence of side information is critical to obtain a non-trivial recovery rate. We then show how to adapt this algorithm to tree decompositions of edge-subgraphs of certain graph families such as lattices, resulting in optimal recovery error rates that can be obtained efficiently The thrust of our analysis is to 1) use the tree decomposition along with edge measurements to produce a small class of viable vertex labelings and 2) apply an analysis influenced by statistical learning theory to show that we can infer the ground truth from this class using vertex measurements. We show the power of our method in several examples including hypergrids, ring lattices, and the Newman-Watts model for small world graphs. For two-dimensional grids, our results improve over Globerson et al. (2015) by obtaining optimal recovery in the constant-height regime.

==> extensions.tex <==
\dfcomment{daniel: remove}
\paragraph{Semi-random model}
Our tree decomposition based approach readily extends to the following semi-random model: Each edge is marked independently with probability $p$. For unmarked edges $(u,v) \in E$ we are provided withthe ground truth labeling $Y_u \cdot Y_v$. For marked edges, an adversary is allowed to arbitrarily set labels. For the noisy vertex labels we assume the same random model as in \pref{mod:edge_vertex_measurement}. 

All our results (e.g. \pref{theorem:main_simple}) immediately extend to this setting with the same rates. To see this, observe that if \pref{lem:extended_component_estimator} and \pref{lem:concentration_extended} hold in the semi-random setting, then the rest of the analysis can be used unchanged. Now \pref{lem:extended_component_estimator} holds for the semi-random setting for any arbitrary labeling of marked nodes within each component and its extension. This is because the lemma only depends on bounding probability that more than half the edges in a cut are flipped, and does not depend on \emph{how} marked edges are relabeled. To prove the \pref{lem:concentration_extended} in the semi-random setting, we move to an upper bound by allowing edges that appear in multiple components to be labeled differently across components (we can have inconsistent labelings). That is, for each component we consider adversarial labelings local to that component and then use the same concentration result used to prove the bound in \pref{lem:concentration_extended}. 

This observation shows that side information enables tight recovery in the semi-random setting. It should be noted that more common inference methods for the pure edge recovery setting such as spectral algorithms often are not robust to semi-random measurements.

\paragraph{General Sub-Algorithms}
While \pref{alg:decoder} considers components of constant size and we use a brute-force algorithm to make inference in each component using edge labels, a careful look at our proof technique reveals that one can replace inference within each component by any arbitrary sub-algorithm (e.g. spectral) that obtains exact recovery within each component up to sign (with bounded failure probability). Thus, our decomposition methodology can be used at a high level to combine different inference techniques (based on edge labels) within each components. This approach can apply even when components are allowed to have super-constant size, and suggests an interesting avenue for exploring computational-statistical tradeoffs.
We remark that even for the brute force enumeration scheme we use in each component, though we currently assume constant size components, we can easily still produce polynomial time algorithms if the component sizes are allowed to be of order $\log n$.
